Symplectic Foliations, Currents, and Local Lie Groupoids

This thesis treats two main topics: calibrated symplectic foliations, and local Lie groupoids. Calibrated symplectic foliations are one possible generalization of taut foliations of 3-manifolds to higher dimensions. Their study has been popular in recent years, and we collect several interesting results. We then show how de Rham's theory of currents, and Sullivan's theory of structure currents, can be applied in trying to understand the calibratability of symplectic foliations. Our study of local Lie groupoids begins with their definition and an exploration of some of their basic properties. Next, three main results are obtained. The first is the generalization of a theorem by Mal'cev. The original theorem characterizes the local Lie groups that are part of a (global) Lie group. We give the corresponding result for local Lie groupoids. The second result is the generalization of a theorem by Olver which classifies local Lie groups in terms of Lie groups. Our generalization classifies, in terms of Lie groupoids, those local Lie groupoids that have integrable algebroids. The third and final result demonstrates a relationship between the associativity of a local Lie groupoid, and the integrability of its algebroid. In a certain sense, the monodromy groups of a Lie algebroid manifest themselves combinatorially in a local integration, as a lack of associativity.

==> chapters/dedication.tex <==
\clearpage
\thispagestyle{plain}
\phantomsection
%\addcontentsline{toc}{chapter}{Dedication}

\vspace*{.35\textheight}
\begin{center}
\large\itshape to my parents
\end{center}


==> chapters/titlepage.tex <==

\thispagestyle{empty}
\makeatletter
\begin{tikzpicture}[remember picture, overlay]
    %\draw (current page.north) -- (current page.south);
    \node[anchor=north,align=center] at ($(current page.north) + (0, -2in)$) {\textsc{\@title}};
    \node[anchor=north,align=center] at ($(current page.north) + (0, -3.5in)$) {\textsc{by} \\ \\ \textsc{\@author}};
    \node[anchor=north,align=center] at ($(current page.north) + (0, -5.5in)$) {\textsc{DISSERTATION} \\ \\ Submitted in partial fulfillment of the requirements \\ for the degree of Doctor of Philosophy in Mathematics \\ in the Graduate College of the \\ University of Illinois at Urbana-Champaign, 2018};
    \node[anchor=north,align=center] at ($(current page.north) + (0, -7.5in)$) {Urbana, Illinois};
    \node[anchor=north west,align=left] at ($(current page.north west) + (1in, -8in)$) {Doctoral Committee: \\ \\
        \hspace*{0.5in} Professor Susan Tolman, Chair \\
        \hspace*{0.5in} Professor Rui Loja Fernandes, Advisor\\
        \hspace*{0.5in} Professor Ely Kerman \\
        \hspace*{0.5in} Professor James Pascaleff };
\end{tikzpicture}
\makeatother


